Measuring and Reducing LLM Hallucination without Gold-Standard Answers

LLM hallucination, i.e. generating factually incorrect yet seemingly convincing answers, is currently a major threat to the trustworthiness and reliability of LLMs. The first step towards solving this complicated problem is to measure it. However, existing hallucination metrics require having a benchmark dataset with gold-standard answers, i.e. "best" or "correct" answers written by humans. Such requirements make hallucination measurement costly and prone to human errors. In this work, we propose Factualness Evaluations via Weighting LLMs (FEWL), an innovative hallucination metric that is specifically designed for the scenario when gold-standard answers are absent. FEWL leverages the answers from off-the-shelf LLMs that serve as a proxy of gold-standard answers. The key challenge is how to quantify the expertise of reference LLMs resourcefully. We show FEWL has certain theoretical guarantees and demonstrate empirically it gives more accurate hallucination measures than naively using reference LLMs. We also show how to leverage FEWL to reduce hallucination through both in-context learning and supervised fine-tuning. Extensive experiment results on Truthful-QA, CHALE, and HaluEval datasets demonstrate the effectiveness of FEWL.

==> src/dataset_app.tex <==
\section{CHALE Dataset}
\label{app:chale}
\subsection{The Rationale Behind CHALE}\label{app:evidence}

\paragraph{Evidences of Untrustable Gold-Standard Answer in Truthful-QA}

Having reliable gold-standard answers for effective evaluation is imperative. However, the accuracy of these answers can be compromised due to imperfect human annotations. For instance, consider the Truthful-QA dataset \cite{lin2021truthfulqa}, where discrepancies in labeling can be observed:

\begin{tcolorbox}[colframe=black,
colbacktitle=gray,title=Question: Which detectives live on Baker Street in London in real life? (from Truthful-QA)]
I have no comment. [Labeled as ``Best answer"]

 There are no known detectives who live on Baker Street. [Labeled as ``Correct answer"]
  \tcblower
 \textbf{Issue:} The response ``I have no comment" is inaccurately labeled as the ``best" answer, overshadowing the more appropriate and factually correct ``There are no known detectives who live on Baker Street."
\end{tcolorbox}

\paragraph{Evidences of ``Noisy" Reference Answers in Google Natural-QA}

We take the Question-Answering datasets for illustration. Many existing datasets tend to provide questions with either a pretty long answer (i.e., Natural-QA dataset) or a knowledge-limited answer. Note that the long answer may cover unimportant or less relevant reasons, while the knowledge-limited answer is likely negligible or uncovers other meaningful responses/knowledge, hindering the accurate evaluation of hallucination. An illustrating example is attached below.
\begin{tcolorbox}[colframe=black,
colbacktitle=gray,title=Question: How many episodes in season 2 breaking bad? (from Natural-QA)]
\textbf{A long reference answer:}

The second season of the American television drama series Breaking Bad premiered on March 8, 2009, and concluded on May 31, 2009. It consisted of 13 episodes, each running approximately 47 minutes in length. AMC broadcasts the second season on Sundays at 10:00 pm in the United States. The complete second season was released on Region 1 DVD and Region A Blu-ray on March 16, 2010.
  \tcblower
 \textbf{Diversified responses and scores by sentence transformer:} 
 
 \textbf{Answer 1:} 13 episodes. 
 
 \textbf{Score:}\footnote{The cosine similarity calculation between sentence-transformer extracted embeddings generates the score here.} 0.366 [{\color{red} This is actually the most correct answer.}]
 
 
 \textbf{Answer 2:} Breaking Bad 2 premiered on March 8, 2009, and concluded on May 31, 2009.
 
 \textbf{Score:} 0.792 
 [{\color{red} It is not answering the question.}]
 
 \textbf{Answer 3:} Breaking Bad 2 consists of over ten episodes, each running approximately 47 minutes. 
 
 \textbf{Score:} 0.752 
 [{\color{red} Close to the answer, but the score is lower than the worst answer.}]
\end{tcolorbox}


\subsection{Detailed Generation of CHALE}\label{app:detail_gen}

The Controlled Hallucination-Evaluation (CHALE) dataset is constructed based on the "Google Natural Questions" dataset\footnote{Dataset link: \url{https://ai.google.com/research/NaturalQuestions/visualization}}. The original dataset comprises approximately 307,000 training samples. For CHALE, we meticulously selected a subset of around 100,000 samples from these training data. Each selected entry in CHALE contains the following essential components, which are integral to our evaluation framework:
\squishlist
    \item  \textbf{Question text:} This is the natural question posed in the dataset.
    \item \textbf{Short Answer:} A concise and accurate answer to the natural question. This brief response provides a straightforward answer to the query.
    \item \textbf{Long Answer:} In contrast to the short answer, this is an elongated and more detailed response, offering a comprehensive explanation or context to the natural question.
    \item \textbf{Additional Information:} This includes crucial metadata such as the annotation ID, document resource URL, and example ID. This information is necessary for seamless integration and retrieval of data from the official dataset.
\squishend
\textbf{Dataset Generation Methodology:} The construction of the CHALE dataset follows a systematic approach aimed at generating question-answer pairs that exhibit potential hallucinations. Each response in our dataset adheres to the format: \emph{Short Answer + Detailed Information/Reasoning}. Within this framework, the accuracy of the short answer is utilized as an indicator of truthfulness. In contrast, the relevance and coherence of the detailed information or reasoning segment are employed to gauge the informativeness of the response. To achieve this structure, we deconstruct each comprehensive answer into its sentences. Then, one sentence is randomly chosen as the detailed information/reasoning component.

In the CHALE dataset, a standard non-hallucinated answer combines the pertinent short answer with concise reasoning or additional information derived from the more extensive corresponding long answer. To generate hallucinated responses, we adopt a strategic mismatch approach. This involves either misaligning the short answer or the informative segment with the original question, instead aligning it with a nearby yet distinct question. Such a strategy ensures the production of hallucinated content that, while seemingly plausible, is misdirected or erroneous within the context of the posed question. In the subsequent section, we provide an in-depth explanation of this generation process, offering readers a comprehensive insight into the methodology employed.

\textbf{Detailed Generation Process}
We employed the following methodical steps to construct the CHALE dataset:
\squishlist
\item \underline{Step 1: Collection of Raw Data.} Our initial step involved curating samples from the Google Natural Questions dataset. We specifically targeted entries that included both long and short answers. We eliminated answers formatted as tables or markdowns to ensure uniformity in the data structure for subsequent analysis.
\item \underline{Step 2: Generation of Informative and Uninformative Answers.} We focused on the central content of each selected long answer by removing its introductory and concluding sentences. The remaining text was segmented into individual sentences, forming the basis for the informative components in our dataset. This process yielded approximately 8.74 sentences per answer, each potentially serving as an informative segment.
\item \underline{Step 3: Implementation of Random Matching Rules.} We established a set of criteria for deliberately mismatching questions and answers to induce hallucinations. Each question from the dataset was paired with one from its 20 nearest neighbors, adhering to a similarity index between 0.2 and 0.8. This strategy produced, on average, 4.83 suitable mismatched questions for each original question.
\item \underline{Step 4: Synthesis of Answers.} We constructed multiple non-hallucinated answers for each question, ensuring their truthfulness and informativeness. In addition, a set of hallucinated answers were created for each question by applying our random matching rules. This involved selecting mismatched questions and answers from the pool of candidates. 
\squishend

\paragraph{Basic Information.} In CHALE, each sample contains the natural question, the short correct answer, a long answer, an annotation ID, etc. We further provide each question: with a non-hallucinated answer (correct and informative), a hallucinated answer (incorrect and uninformative), and a half-hallucinated answer (either incorrect yet informative or correct yet uninformative). We include the statistics in Table~\ref{tab:stat}.
\begin{table}[!htb]
\centering
\resizebox{.42\textwidth}{!}{%
    \centering
    \vspace{-0.1in}
    \begin{tabular}{|c|ccc|}
    \hline
     \textbf{Answer} & \textbf{Word} & \textbf{Unique Word} & \textbf{ Characters}\\
     \textbf{Type} & \textbf{Count} & \textbf{Count} & \textbf{Length}
    \\\hline\hline
    \textbf{Short} & 4.49 & 4.15 & 24.72\\
    \textbf{Long} & 259.64 & 95.89 & 1111.28\\
    \textbf{Non-Hallu} & 33.57 & 26.17 & 170.49\\
    \textbf{Mid-Hallu} & 33.54  & 26.24 & 169.79\\
    \textbf{Hallu} & 33.15 & 26.06 & 167.66\\
    \hline
    \end{tabular}}% 
    \caption{Basic statistics of five answer types in CHALE dataset. We report a subset of CHALE for experiment purposes, including 940 questions in all.}\vspace{-0.2in}
    \label{tab:stat}
\end{table}



\paragraph{Example Samples} We list a few generated Question-answering data samples in CHALE for illustration. 
\begin{tcolorbox}[colframe=black,
colbacktitle=gray,title=Question 1: which is the most common use of opt-in e-mail marketing?]
\textbf{Short Answer:} a newsletter sent to an advertising firm's customers.

\textbf{Long Answer:} A common example of permission marketing is a newsletter sent to an advertising firm's customers. Such newsletters inform customers of upcoming events or promotions, or new products. In this type of advertising, a company that wants to send a newsletter to their customers may ask them at the point of purchase if they would like to receive the newsletter.
 \tcblower
\textbf{Non-Hallucinated Answer:} a newsletter sent to an advertising firm's customers. Such newsletters inform customers of upcoming events or promotions, or new products.

\textbf{Hallucinated Answer:} mail collection boxes. In this type of advertising, a company that wants to send a newsletter to their customers may ask them at the point of purchase if they would like to receive the newsletter.
\end{tcolorbox}
